Towards an Automated Requirements-driven Development of Smart Cyber-Physical Systems

The Invariant Refinement Method for Self Adaptation (IRM-SA) is a design method targeting development of smart Cyber-Physical Systems (sCPS). It allows for a systematic translation of the system requirements into the system architecture expressed as an ensemble-based component system (EBCS). However, since the requirements are captured using natural language, there exists the danger of their misinterpretation due to natural language requirements' ambiguity, which could eventually lead to design errors. Thus, automation and validation of the design process is desirable. In this paper, we (i) analyze the translation process of natural language requirements into the IRM-SA model, (ii) identify individual steps that can be automated and/or validated using natural language processing techniques, and (iii) propose suitable methods.

==> eptcsdata.tex <==
\providecommand{\firstpage}{59}
\providecommand{\publicationstatus}{J. Kofro\v{n}, J. Tumova, B. Buhnova (Eds.): Formal Engineering\\
Approaches to Software Components and Architectures (FESCA'16)\\
EPTCS 205, 2016, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.205.5}{10.4204/EPTCS.205.5}}
\pdfoutput=1

